Addressing Uncertainty in LLMs to Enhance Reliability in Generative AI

In this paper, we present a dynamic semantic clustering approach inspired by the Chinese Restaurant Process, aimed at addressing uncertainty in the inference of Large Language Models (LLMs). We quantify uncertainty of an LLM on a given query by calculating entropy of the generated semantic clusters. Further, we propose leveraging the (negative) likelihood of these clusters as the (non)conformity score within Conformal Prediction framework, allowing the model to predict a set of responses instead of a single output, thereby accounting for uncertainty in its predictions. We demonstrate the effectiveness of our uncertainty quantification (UQ) technique on two well known question answering benchmarks, COQA and TriviaQA, utilizing two LLMs, Llama2 and Mistral. Our approach achieves SOTA performance in UQ, as assessed by metrics such as AUROC, AUARC, and AURAC. The proposed conformal predictor is also shown to produce smaller prediction sets while maintaining the same probabilistic guarantee of including the correct response, in comparison to existing SOTA conformal prediction baseline.

==> background.tex <==
\section{Background}
\label{sec:bkgrnd}

\subsection{Conformal Prediction and Inductive Conformal Prediction}
Conformal prediction (CP)~\citep{cp,icp} is a general framework for generating valid prediction sets by prediction models such as DNN classifiers. A prediction set is more useful than a point prediction for quantifying the uncertainty in the output of a predictive model. A valid prediction set is one that contains the true label with a high probability.

For the given set  $X=\{x_i : 1 \leq i \leq l\}$ and a new input $x_{l+1}$, CP generates a prediction set $\Gamma^{\epsilon}_{l+1}$ for the label $y_{l+1}$ of $x_{l+1}$. The prediction set is valid as the probability of $\Gamma^{\epsilon}_{l+1}$ containing the true label for $x_{l+1}$ is greater than or equal to $1$ minus the significance level  $\epsilon$: $Pr(y_{l+1} \in \Gamma^{\epsilon}_{l+1}) \geq 1-\epsilon,$ under the assumption the $x_1,\ldots,x_{l},x_{l+1}$ are exchangeable. 

The core idea of CP is to compute a $p$-value of the input w.r.t to each possible label of $x_{l+1}$, and include all those labels $y$ in the prediction set whose $p$-value ($p^y_{l+1}$) is greater than or equal to $\epsilon$:
\begin{equation*}
    \Gamma^{\epsilon}_{l+1} = \{y \ | \ p^{y}_{l+1} > \epsilon\}.
\end{equation*}

A Non-Conformity Measure (NCM) is used for computing these $p$-values. An NCM is a real-valued function $\mathcal \mathcal{A}(X,x)$ that assigns a non-conformity score $\alpha$ to $x$ relative to datapoints in the training set $X$. An example of the NCM for a DNN classifier is the normalized distance of $x \in X$ from its  nearest neighbor in the training set $X$ with the same label:
\begin{equation*}
    \alpha_i = \frac{min_{j=1,\ldots,l:j\neq i \& y_j=y_i}Dis(x_i,x_j)}{min_{j=1,\ldots,l:y_j \neq y_i}Dis(x_i,x_j)},
\end{equation*}
where $Dis$ is the distance metric defined on $X$ (Intuitively, an example conforms to the sequence if it
is close to the other examples with the same label and far from the examples with
a different label). 

For a new input $x_{l+1}$, we can compute $\alpha^{y}_{l+1}$ for each $y\in Y$, and create the prediction set with all those labels whose $p^{y} > \epsilon$, where $p^{y}$ is calculated as follows:

\begin{equation*}
    p^{y} = \frac{|\{i=1,...,l\}: \alpha_i \geq \alpha^{y}|+1}{l+1}.
\end{equation*}

Apart from the distance between nearest neighbors~\citep{icp}, other examples of previously proposed NCM are based on ridge regression~\citep{icp}, support vector machines~\citep{icp}, random forests~\citep{ncm-rf}, VAE and SVDD~\citep{vanderbilt}. An example of the most commonly used NCM for DNN regressors is the absolute difference between the true value and the predicted value by the regressor trained on $X$. %Add details about the prediction region - maybe Quantile CP here. (say, although we have used classifier as an example)

The training set is updated with the label of the current test input $x_{l+1}$ before predicting the label of the next input. For every new datapoint, re-calculating $\alpha_i$ based from NCM on the updated training set (last training set appended with the last test input) might become computationally infeasible if evaluating the underlying NCM $\mathcal \mathcal{A}$ is expensive. To resolve this issue, inductive conformal prediction (ICP)~\citep{icp} was introduced.  

In ICP, the training set is split into a \textit{proper training set} $X_{\text{tr}} = \{x_i: i=1,\ldots,m\}$ and a \textit{calibration set} $X_{\text{cal}}=\{x_j: j=m+1,\ldots,l\}$. Further, the non-conformity scores for each datapoint $x_j \in X_{\text{cal}}$ and the new datapoint $x_{l+1}$ are calculated relative to the proper training set:
\begin{equation*}
    \alpha_j = \mathcal \mathcal{A}(X_{\text{tr}}, x_j)
    \qquad \text{and} \qquad
    \alpha_{l+1} = \mathcal \mathcal{A}(X_{\text{tr}}, x_{l+1}).
\end{equation*}
% And $p$-value for a label $y$ of the input $x_{l+1}$ is computed by comparing its non-conformity score with these scores for the calibration set:

% \begin{equation*}
%     p^{y} = \frac{|\{i=1,...,m+1\}: \alpha_i \geq \alpha^{y}|+1}{l-m+1}.
% \end{equation*}

The prediction set includes all those labels, whose non-conformity score lies in the $(1-\epsilon)^{th}$ quantile of the empirical distribution of the non-conformity scores for the calibration set. Specifically, all those labels are included in the prediction set whose score is less than or equal to the $q=\lceil (l-m+1)(1-\epsilon) \rceil^{th}$ smallest non-conformity score of the calibration set. 

ICP retains the validity of the CP framework, i.e., the probability of the true label lying in the predicted set by ICP is greater than or equal $1-\epsilon$. This assumes that the datapoints in $X_{cal}$ and $x_{l+1}$ are i.i.d given the proper training set $X_{tr}$, and therefore the corresponding non-conformity scores are also exchangeable.
